Self-Consistent Spin, Tidal and Dynamical Equations of Motion in the REBOUNDx Framework

We have introduced self-consistent spin, tidal and dynamical equations of motion into REBOUNDx, a library of additional effects for the popular N-body integrator REBOUND. The equations of motion used are derived from the constant time lag approximation to the equilibrium tide model of tidal friction. These effects will allow the study of a variety of systems where the full dynamical picture cannot be encapsulated by point particle dynamics. We provide several test cases and benchmark the code's performance against analytic predictions. The open-source code is available in the most recent release of REBOUNDx.

==> reviewer_response.tex <==
L263: Both these limiting cases: Authors could be more clear and mention again these limiting cases.

The helper function itself has since been removed, but we now explicitly mention when this relation is valid in line 265

L 299: Moment of Inertia : "I" is used later but I am not sure whether the dimensionless moment of inertia C is referenced later in the paper.

C is referenced again - in both sections 5.1 (line 498) & 5.3 (line 644)

L370: Possible rage of values (or some examples) for the dissipation constant (also Love Number k?) could be discussed further briefly with some references. Is the code working with any range of values dissipation constant or are there some limits? Also the units could be given when it is introduced (see L370, L576 ) ? Can the dissipation be considered time dependent ?

In each of the examples in section 5, fiducial values for all additional parameters are given along with references. We have since restructured the code to be in terms of the constant time lag tau rather than sigma using Equation (1). The code is valid for any range of sigma/tau, and this quantity is intrinsic to each body. This has been explicitly stated in line 188. Time dependence is not supported officially at the moment -  the user can manually change the parameters at a given time if they wish, but nothing more sophisticated exists at the moment.

Figure 2: left subplot, numbers missing in X axis

The X axis is shared between the upper and lower subplots.

In addition to these changes, minor edits reflect some changes in code syntax made post-submission. This does not affect any of our results.
